Scale invariant transfer matrices and Hamiltionians

Given a direct system of Hilbert spaces $s\mapsto \mathcal H_s$ (with isometric inclusion maps $\iota_s^t:\mathcal H_s\rightarrow \mathcal H_t$ for $s\leq t$) corresponding to quantum systems on scales $s$, we define notions of scale invariant and weakly scale invariant operators. Is some cases of quantum spin chains we find conditions for transfer matrices and nearest neighbour Hamiltonians to be scale invariant or weakly so. Scale invariance forces spatial inhomogeneity of the spectral parameter. But weakly scale invariant transfer matrices may be spatially homogeneous in which case the change of spectral parameter from one scale to another is governed by a classical dynamical system exhibiting fractal behaviour.

==> d=2.4 <==
#FIG 3.2  Produced by xfig version 3.2.5b
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 5775 4575 6225 5025
2 1 0 5 4 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5850 4650 6150 4950
2 1 0 5 4 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5850 4950 6150 4650
-6
6 3450 375 3900 825
2 1 0 5 2 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3525 450 3825 750
2 1 0 5 2 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3525 750 3825 450
-6
1 3 0 0 0 1 50 -1 20 0.000 1 0.0000 7350 5100 75 75 7350 5100 7425 5100
1 3 0 0 0 6 50 -1 20 0.000 1 0.0000 3225 525 75 75 3225 525 3300 525
2 1 0 3 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	2 1 4.00 60.00 120.00
	 225 4800 12225 4800
2 1 0 5 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2475 4725 2475 4875
2 1 0 5 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9525 4725 9525 4875
2 1 0 3 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	2 1 4.00 60.00 120.00
	 6000 9600 6000 0
2 1 0 5 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 -2025 7425 -2175
2 1 0 5 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5925 600 6075 600
2 1 0 5 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5925 9000 6075 9000
2 2 0 0 5 5 50 -1 20 0.000 0 0 -1 0 0 5
	 1350 3150 1500 3150 1500 3300 1350 3300 1350 3150
2 2 0 0 5 5 50 -1 20 0.000 0 0 -1 0 0 5
	 600 8100 750 8100 750 8250 600 8250 600 8100
2 2 0 0 5 5 50 -1 20 0.000 0 0 -1 0 0 5
	 3675 4650 3825 4650 3825 4800 3675 4800 3675 4650
2 2 0 0 5 5 50 -1 20 0.000 0 0 -1 0 0 5
	 4575 7350 4725 7350 4725 7500 4575 7500 4575 7350
2 2 0 0 5 5 50 -1 20 0.000 0 0 -1 0 0 5
	 5325 2400 5475 2400 5475 2550 5325 2550 5325 2400
3 0 1 3 0 5 50 -1 -1 8.000 0 1 0 4
	0 0 3.00 120.00 120.00
	 6075 5025 6450 5325 6900 5325 7200 5175
	 0.000 1.000 1.000 0.000
3 0 1 3 0 5 50 -1 -1 8.000 0 1 0 4
	0 0 3.00 120.00 120.00
	 5700 4725 3150 3150 2625 1200 3150 600
	 0.000 1.000 1.000 0.000
3 0 1 3 0 5 50 -1 -1 8.000 0 1 0 4
	0 0 3.00 120.00 120.00
	 3675 450 3525 225 3375 225 3225 450
	 0.000 1.000 1.000 0.000
3 0 1 3 0 5 50 -1 -1 8.000 0 1 0 5
	0 0 3.00 120.00 120.00
	 3750 600 5550 1425 8025 3750 7725 4500 7350 5100
	 0.000 1.000 1.000 1.000 0.000
3 0 1 3 11 5 50 -1 -1 8.000 0 1 0 5
	0 0 3.00 60.00 120.00
	 3000 525 2100 750 1650 1425 1500 2625 1425 3150
	 0.000 1.000 1.000 1.000 0.000
3 0 1 3 11 5 50 -1 -1 8.000 0 1 0 6
	0 0 3.00 60.00 120.00
	 7350 5175 6900 6000 3675 6375 1350 5325 1050 4200 1425 3300
	 0.000 1.000 1.000 1.000 1.000 0.000
4 0 0 50 -1 3 20 0.0000 4 225 150 9375 5400 1\001
4 0 0 50 -1 3 20 0.0000 4 225 255 2325 5325 -1\001
4 0 0 50 -1 3 30 0.0000 4 225 195 6150 300 r\001
4 0 0 50 -1 3 20 0.0000 4 225 255 6225 9075 -1\001
4 0 0 50 -1 3 20 0.0000 4 225 315 6300 675 +1\001

